Decidable Logics Combining Word Equations, Regular Expressions and Length Constraints

In this work, we consider the satisfiability problem in a logic that combines word equations over string variables denoting words of unbounded lengths, regular languages to which words belong and Presburger constraints on the length of words. We present a novel decision procedure over two decidable fragments that include quadratic word equations (i.e., each string variable occurs at most twice). The proposed procedure reduces the problem to solving the satisfiability in the Presburger arithmetic. The procedure combines two main components: (i) an algorithm to derive a complete set of all solutions of conjunctions of word equations and regular expressions; and (ii) two methods to precisely compute relational constraints over string lengths implied by the set of all solutions.We have implemented a prototype tool and evaluated it over a set of satisfiability problems in the logic. The experimental results show that the tool is effective and efficient.

==> algo-flaten.tex <==
 \begin{algorithm2e}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$(\se_r, \se_i)$} \Output{$(\var_i,\production_i)$}
$\traces_{cyc} \leftarrow \code{cycles}(\se_r, \se_i) $\tcc*{sequence of all cycles in top-down order}
$\sub_{noncyc} \leftarrow \code{labels}(\se_r, \se_i) $\tcc*{substitutions not in any cycle}
 $\var_i \leftarrow \code{vars}(\se_r, \se_i)$\tcc*{set of all variables}
  $\production_i \leftarrow \emptyset $\;
\ForEach { $v_j \in \var_i$}
{
   $v_{run} \leftarrow  v_j $\;
  \ForEach { $\vtree{\se_c}{\se_b}{\sub_{cyc}}{v_j}$ $\in \traces_{cyc}$}
  {
    $v_{next} \leftarrow  v_{fresh} $ \tcc*{ symbol for next stage}
    $\vtree{\se_c}{\se_b}{\sub_{cyc}}{v_j} {\leftarrow} \ulabels{\vtree{\se_c}{\se_b}{\sub_{cyc}}{v_j}}{[v_{run}/v_j]}$\;
    $\production_i  \leftarrow \production_i \cup \{(v_{run}, v_{next})\} $ \tcc*{production rule to connect cycles}
    $v_{run} \leftarrow   v_{next} $\;
  }
  \If{$(v_{run} \not= v_{j}) $}{
    $\sub_{noncyc} {\leftarrow} \ulabels{\sub_{noncyc}}{[v_{run}/v_j]}$\;
  }
}
\ForEach { $\ctree{\se_c}{\se_b}{\sub_{cyc}}$ $\in \traces_{cyc}$}
  {
$\production_i  \leftarrow \production_i \cup \bigcup \{(s_1,s_2) \mid [s_2/s_1] \in \clabel{\ctree{\se_c}{\se_b}{\sub_{cyc}}}  \} $ \tcc*{each cycle}
}
  $\production_i  \leftarrow \production_i \cup \bigcup \{(s_1,s_2) \mid [s_2/s_1] \in \sub_{noncyc}  \} $ \tcc*{non-cycle}
 \Return{$(\var_i, \production_i)$};

\caption{Procedure $\code{\extractaux}$}\label{algo.ftree}
\end{algorithm2e}


==> algo-graph.tex <==
% \begin{figure}[tbh]
 %% \begin{center}
 %% \begin{minipage}{0.98\textwidth}
 % \begin{frameit}

 \begin{algorithm2e}[t]
%%\begin{procedure}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$ \se$} \Output{\utree{n}}
   $i {\leftarrow} 0 $; %% $\sstate^{comp} {\leftarrow} \{ \}$;
   %% $\sstate {\leftarrow} \{ \ind \}$ \tcc*{initialize}
    $\se_0 {\leftarrow} \matchse(\se)$;
   $\utree{0} {\leftarrow} \se_0$ \tcc*{initialize}
 \While { $\true$ }
 {
      $\utree{i} {\leftarrow} \code{\eval}(\utree{i})  $ \tcc*[r]{check unsat/sat and mark closed}
      $ \utree{i}  {\leftarrow} \code{\lb}(\utree{i}) $ \tcc*[r]{detect similarly}
      $(\code{is\_exists}, \se_i) {\leftarrow} \code{choose}(\utree{i})  $ \tcc*[r]{ leaf for next reduction}
      \uIf{ not~ \code{is\_exists}}{
       \Return{{{\utree{i}}}} \tcc*[r]{cyclic tree}
     }\Else{
        $ i {\leftarrow} i{+}1 $ \;
       $ \utree{i}  {\leftarrow} \code{reduce}(\se_i) $ \tcc*[r]{reduced with arrangements}
      }
 }
 \caption{{\allSat}.}\label{algo.graph}
\end{algorithm2e}
%\savespace
%\end{figure}


==> cfg-correct.tex <==
%% for CFG
We show that each production relation derived
is satisfied to construct a CFG.

\begin{lemma}\label{extractcfg.prod}
Let \form{\mtree{\se_c}{\se_b}{\sub_{cyc}}} be a cyclic reduction tree
derived by {\allSat}. \form{\sub_{cyc}} is of the form: \form{[X'/X]},
where \form{X} and \form{X'} are two string variables.
\end{lemma}

\begin{proof}

\qed
\end{proof}

\begin{lemma}
Let \form{(\tnode_1,\sub,\tnode_2)}
is an edge in a cyclic reduction tree derived by {\allSat}.
Then, either  \form{\sub{\equiv}[tr/X]} where \form{X} is a string variable.
\end{lemma}
\begin{proof}

\qed
\end{proof}

%%\input{min-tree-contra}


\begin{thm}
Suppose that \form{\se} is a quadratic word equation,
\form{\allSat(\se)} derives for \form{\se}  a  cyclic reduction tree
\form{\utree{n}} in a finite number of iterations, and
\form{\extractcfg(\utree{n})} produces a set of CFG
\form{\cfgs} in finite time.
Then,
\begin{enumerate}
\item \form{\cfgs} is a set of CFG.
\item Let \form{G} be the union of all CFG in \form{\cfgs}.
The language produced by \form{G}
represents all solutions of \form{\se}.
\end{enumerate}
\end{thm}

Secondly, we prove the termination of \form{\extractcfg}.
\begin{proposition}[{\extractcfg} Termination]\label{lemma.extractcfg.term}
Suppose that \form{\utree{i}} is a cyclic reduction tree derived by
{\allSat} for a quadratic word equation.
{\extractcfg} terminates for \form{\utree{i}}.
\end{proposition}
\begin{proof}
This termination is based on the 
fact that
there are finite number of cycles in \form{\utree{i}}.
\qed
\end{proof}

%% \paragraph{Procedure {\secfg}} The termination of 
%% {\secfg} follows from the termination of sub-procedure {\allSat}
%% (lemma \ref{lemma.allsat.term}) and the fact that
%% there are finite number of cycles in every cyclic reduction trees
%% which {\allSat} constructs for quadratic word equations.
\begin{thm}\label{algo.term}
{\secfg} terminates for
 quadratic word equations.
\end{thm}
\begin{proof}
This theorem immediately follows from Prop. \ref{lemma.allsat.term}
and Prop. \ref{lemma.extractcfg.term}.
\qed
\end{proof}



==> cfg-sem.tex <==


\begin{defn}[\form{\strcfsem} Formulas]
The normalized formula
 \form{\pure_{\strcf}{\equiv} \se{\wedge} \astart{\wedge}\ariths}
is called in the \form{\strcfsem} %% decidable
fragment
if {\allSat} take \form{\se} as input,
and produces a cyclic reduction tree  \form{\utree{n}}
  in a finite time. Furthermore,
any cycle \form{\ctree{\se_c}{\se_b}{\sub_{cyc}}}
 of \form{\utree{n}}, both two following properties hold:
\begin{itemize}
\item The labels along the path (\form{\se_c}, \form{\se_b})
 (assume that this
 path has \form{k} edges) is of the form:
\form{[y_1X_1/X]}, \form{[y_2X_2/X_1]},..., \form{[y_{k+1}X_{k+1}/X_{k}]}
where \form{X}, \form{X_i} (\form{i \in \{1,...,k+1 \}}) are string
variables
and \form{y_i} (\form{i \in \{1,...,k+1 \}}) is either a string
variable or a letter.
\item The substitution \form{\sub_{cyc}= [X/X_{k+1}]}.
\end {itemize}
\end{defn}
We refer the variable \form{X} as an extensible variable
and such cycle as \form{\vtree{\se_c}{\se_b}{\sub_{cyc}}{X}}.
Furthermore, we use \form{\clabel{\vtree{\se_c}{\se_b}{\sub_{cyc}}{X}}}
to return a sequence of substitutions
 of the cycle (including the substitution of the back link) (e.g.,
\form{\clabel{\vtree{\se_c}{\se_b}{\sub_{cyc}}{X}}=} \form{\{y_1X_1/X,y_2X_2/X_1,...,} \form{[y_{k+1}X_{k+1}/X_{k},X/X_{k+1} \}}).

For a, decision procedure over this fragment,
we revise {\deci} by replacing procedure
{\extractedtl} at line 4 (Fig. \ref{algo.sat})
by procedure {\extractcfg}.
Procedure {\extractcfg} and its correctness is described in
the next subsection.


==> cfg-syn-complexity.tex <==

\paragraph{Complexity of {\allSat}}
Our analysis relies on the following lemmas
which show that the number of edges of a cycle
is at most polynomial.

Let \form{\ctree{\se_c}{\se_b}{\sub_{cyc}}} be a cycle 
with the companion \form{\se_c} 
and the bud \form{\se_b}.
The number of edges of the path from  \form{\se_c} 
to \form{\se_b} is called the length of the cycle.






\begin{lemma}\label{lem.reduce.cycle}
Length of a cycle is less than word equation length.
\end{lemma}

\begin{proof}
One occurrence.

We remark that a cycle is constructed when the equation at the root of the tree
contains at least one variable with two occurrences.

If two occurrences are at the same side

one is in LHS and another is in RHS.
Without loss of general, assume that the companion of a cycle
of variable \form{X} is
\form{X tr_1 = Ytr_2 X}. At the first reduction,
\form{YX_1/X}, \form{X_1 tr_1 = tr_2 YX_1}.  To form a cycle,
at each reduction step, the first term (a variable or a character)
in the LHS
is reduced and matched with the first term in the RHS
until \form{Y} variable is the first term of the RHS.
so, the length of the cycle is equal to \form{N{-}1}.
\end{proof}


\begin{lemma}\label{lem.reduce.min.sol}
Minimal solution is polynomial
\end{lemma}

\begin{proof}
max \form{N/2} cycles

\form{(N/2) \times (N-1) + N}
\end{proof}

\begin{proposition}[{\allSat} Termination]\label{lemma.allsat.term}
{\allSat} terminates for quadratic word equations.
\end{proposition}

\begin{proof}
The correctness of this
 proposition immediately follows from lemmas \ref{lem.reduce.size}
and \ref{lemma.allsat.compl}.
\qed
\end{proof}


==> deci-cfl.tex <==
In this section, we first present \form{\strcf},
 a subfragment of \form{\stredtsem}, in which
the set of all solutions of each word equation
forms a CF language. %% (subsection \ref{sec.dec.cfg.sem}).
 Next, in subsection
\ref{algo.extractcfg} we revise procedure {\deci}
for this fragment
by introducing function {\extractcfg}
to extract CFGs from reduction trees rather than
\form{\edtl} systems.
%% Finally, in subsection \ref{sec.dec.cfg.syn}
%% we syntactically define \form{\strcf},
%% a subfragment of \form{\strcfsem}, where each word equation
%% is both quadratic and twisted.
After that, in subsection \ref{sec.dec.cfg.syn} 
 we syntactically define \form{\strcf},
 a subfragment of \form{\strcfsem}, where each word equation
 is phased-twisted
and also provide analyses on computational complexity
of {\allSat}.
% as well as
%minimal solutions of word equations over this fragment.
Finally, we show how to compute Parikh image of {\cfl}
in subsection \ref{sec.dec.cfg.parikh}.
%\subsection{\form{\strcfsem} Fragment}\label{sec.dec.cfg.sem}
\input{cfg-sem}

%% \subsection{Deriving CFG}\label{algo.extractcfg}
%% \input{tree-2-cfg}


\subsection{\form{\strcf} Fragment}\label{sec.dec.cfg.syn}

\input{cfg-syn}

%% \input{cfg-syn-complexity}


%% \input{cfg-correct}




==> ext.tex <==
\input{norm}


==> fig-cfg.tex <==
%\begin{figure}[ht]
 \begin{algorithm2e}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$\utree{i}$} \Output{$G$}
  $\cfgs_r \leftarrow \emptyset $\; 
 \ForEach {$\se_i \in \code{sat\_leaf(\utree{i})}$}
 {
   $ (\var_i, \production_i) \leftarrow \extractaux(\se_r, \se_i)   $ \tcc*{solutions for one solution path}
    $\var_i \leftarrow \var_i \cup \{S_i\}$;
    $\production_i \leftarrow \production_i \cup \{(S_i, LHS(\se_r))\}$ \tcc*{start symbol and its rule}
   $\cfgs_r {\leftarrow} \cfgs_r \cup \{(\var_i, \alphabet, \production_i, S_i)\}$\;
 }
   \Return{$\bigcup\cfgs_r$} \tcc*{union CFGs}
 \caption{Procedure \code{\extractcfg}}\label{algo.cfg}
\end{algorithm2e}
% \end{figure}


==> fig-match.tex <==
\begin{figure*}[thb]
\begin{center}
%% \savespace
 \begin{minipage}{1\textwidth}
 \begin{frameit}\vspace*{-2.5mm}\savespace
\[
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{CONSTs} \\
\form{\seppredF{\code{STR}}{u{,}0{,}r_u}} \text{ represents } c \qquad
\form{\seppredF{\code{STR}}{v{,}0{,}r_v}} \text{ represents } c  \\
\rho=[0/r_u,0/r_v] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\br'{=} \br {\setminus} \{\myit{i} ~|~ \FV(\myit{i}) {\subseteq} \{r_u,r_v\} \} \\
\code{match}(\satge{\bases'}{\boundaries{\setminus}\{r_u,r_v\}}{\br'}{Inv}) ~{\yields}~{\sge}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u{,}0{,}r_u},\form{\seppredF{\code{STR}}{v{,}0{,}r_v}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\qquad
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{CONST-VAR} \\
\form{\seppredF{\code{STR}}{u{,}0{,}r_u}} \text{ represents } c \qquad
\form{\seppredF{\code{STR}}{v{,}0{,}r_v}} \text{ represents a variable}  \\
\rho=[0/r_u] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\fresh ~v' \quad \br'{=} \br {\setminus} \{\myit{i} ~| \FV(\myit{i}) {\subseteq} \{r_u{,}r_v\} \} \\
{\sge} {=}\satge{\bases'}{\boundaries{\setminus}\{r_u\}}{\br'{\cup}\{r_v{\geq}0 \}}{Inv\subst{v'}{v}{\wedge}v'{=}c{\cdot}v}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u{,}0{,}r_u},\form{\seppredF{\code{STR}}{v{,}0{,}r_v}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\]
\[
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{VARs} \\
\form{\seppredF{\code{STR}}{u_i{,}0{,}r_u}},\form{\seppredF{\code{STR}}{u_{\dual{i}}{,}0{,}r_u}}  \text{ are dual of each another.}  \\
\rho=[0/r_u] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\bases''{=} \bases'{\cup} \{\seppredF{\code{STR}}{v'{,}0{,}r_v} \} \quad
\br'{=} \br {\setminus} \{\myit{i} ~|~ \FV(\myit{i}) {\subseteq} \{r_u\} \} \\
{\sge} {=}\satge{\bases''}{\boundaries{\setminus}\{r_u\}}{\br'{\cup}\{r_v{\geq}0 \}}{Inv{\wedge}u{=}c{\wedge}v{=}c{\cdot}v'}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u_i{,}0{,}d_i},\form{\seppredF{\code{STR}}{u_{\dual{i}}{,}0{,}d_i}, \seppredF{\code{STR}}{t{,}l_t{,}r_t}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\]
\end{frameit}
 \end{minipage}
\caption{Matching Rules}\label{fig.sat.match}
\end{center}
\end{figure*}


==> multi-wordeq.tex <==
\label{sec.mul.eq}
Next, we show a reduction for
multiple word equations.
%% We adapt the approach presented in \cite{khmelevski1976equations}
%% to reduce multiple word equations.
%% This approach is summarized in the following propositions.

%% \begin{proposition}[1.28 \cite{khmelevski1976equations}]
%% For any system of word equations in \form{n}
%% unknowns it is possible to construct a word equation
%% in \form{n} unknowns which is equivalent to the system.
%% \end{proposition}

%% The above proposition was proven based on the following lemma.
%% \begin{lemma}[\cite{khmelevski1976equations}]\label{lemma.eqs}
%% Suppose that \form{X_1}, \form{X_2}, \form{Y_1} and
%% \form{Y_2} are words in \form{\alphabet^*}
%% and
%% \[
%%  \form{X_1{\cdot}a{\cdot}X_2{\cdot}X_1{\cdot}b{\cdot}X_2~{=}~Y_1{\cdot}a{\cdot}Y_2{\cdot}Y_1{\cdot}b{\cdot}Y_2}
%% \]
%%  where \form{a} and \form{b}
%% are distinct characters in \form{\alphabet}.
%% Then, \form{X_1{=}Y_1} and  \form{X_2{=}Y_2}.
%% \end{lemma}
\begin{proposition}
Let \form{a} and \form{b} be distinct letters, \form{a{\neq}b},
and let
 \form{{\pure}{\equiv} l_1{=}r_1{\wedge}...{\wedge}l_k{=}r_k} be
 a conjunction of multiple word equations.
Then the set of solutions of {\pure}
is identical with the set of solutions of the following equation:
 \form{l_1a...l_k a l_1 b ...
l_kb~{=}~r_1 a ...r_k a r_1 b...r_kb}.
\end{proposition}


==> norm-re.tex <==

\cite{Abdulla:CAV:2014}


==> parikh.tex <==
word equations and context-free grammars.

Let \form{G_{x_i}{=}\grammar{\var}{\alphabet}{\production}}

Parikh image \cite{Parikh:JACM:1966}

the main step is 
for each CFG
to generate an existentially quantified  Presburger formula
 which has the same Parikh image.
Our method is based on
the technique presented in \cite{Verma2005}.

\hide{Context-free grammar (CFG) to nondeterministic finite automation (NFAs) 

Parikh equivalent

It is well known that the state cost of the conversion of 
NFA into equivalent deterministic finite automation (DFAs) is
exponential. This means
using the classical subset construction \cite{Rabin:IBM:1959},
we can transform
from each \form{n}-state NFA into an equivalent DFA with \form{2^n} states.

Optimization:
conversion of 
CFG and NFA into Parikh equivalent deterministic finite automation (DFAs)
Parikh \cite{Esparza:IPL:2011} \cite{Lavado:DLT:2012}


DFA to regular expression


regular expression to linear arithmetic
\cite{Esparza:IPL:2011}
\cite{Liang:FroCos:2015}}


==> proof-flat-length.tex <==
\locsay{todo}
\begin{proof}
 we identify recursive predicates through graph dependency.

a predicate is defined either a based formula
or self-recursive formula or a dependent formula.


bottom up to show Presburger-definable.

\cite{Makoto:APLAS:2016}
\end{proof}


==> quad.tex <==
%%for termination




==> review-popl2018 <==
Review #109A
===========================================================================
* Updated: 17 Sep 2017 2:51:21pm EDT

Overall merit
-------------
3. Weak reject - will not argue against

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
This paper presents some nontrivial advances in the problem of solving word equations with length constraints. Word equations are equations over the free-semigroup in which variables are elements of Sigma*. Length constraints are expressed in Presburger arithmetic and can impose restrictions on the length of the string variables. Decidability for the combined logic is open and is perhaps one of the most interesting problems in decision procedures at the moment because it does have practical implications in the analysis of Javascript programs. In fact, several researchers are actively working in this field and many new practical solvers for word equations are appearing. This paper presents an approach for solving equations in such a form that is sound and complete for several fragments of this theory, most remarkably for quadratic word equations (those in which each variable appears at most twice in the system). The algorithm is based on computing a closed form representation
 of the set of solutions and then using Parikh's theorem to compute the lengths of the solutions and find if one satisfies the length constraints. The algorithm is implemented and evaluated against existing tools and it's showed to be effective on the used benchmarks.

Comments for author
-------------------
This paper attacks a really important problem in decision procedures and proposes an algorithm that is based on many nice concepts in formal language theories---e.g., EDT0L languages, Parikh's theorem. In general, the complexity of the tackled problem comes from the fact that there is no easy way to compute the set of lengths of the solutions of arbitrary word equations. This paper shows that for quadratic equations (and for other semantic fragments) this can be done using a nice tree-based representation that only induces EDT0L languages. For such languages, the set of lengths is semi-linear (using an extension Parikh's theorem). The algorithm is implemented in a tool and evaluated against other systems, but the evaluation is completely arbitrary and uses benchmarks of unclear origin. Also, it's unclear whether quadratic word equations are an important fragment in practice from the paper writing. Finally, the paper is full of typos and it's extremely dense. While I could app
 reciate the overall idea, I think the paper needs a major rewriting to clean the presentation. Right now there is a long list of theorems, propositions, and lemmas that make the flow incredibly terse and gave me a very hard time understanding very simple concepts.

PROS:
- Decision procedure for interesting fragment of word equations with length constraints (please address the comments of the expert reviewer).

CONS:
- Writing needs improvement in terms of clarity of presentation and number of typos.
- Evaluation is arbitrary. The authors do not discuss what benchmarks the evaluation was performed and how such benchmarks were obtained.

QUESTIONS FOR AUTHORS:
- Are all the solvers for strings really unsound even when returning SAT? I think CVC4 actually checks whether the produced solution is indeed a model.
- Where are the benchmarks from? The paper doesn't mention any source. Did the eval use classic benchmarks from other papers or are they hand-crafted?

MINOR:
- Lots of typos I'll just point to a few: PSPASE -> PSPACE, This length constrains -> These length constraints, We was -> We were, Plandownki misspelled, automaton is singular vs autoamta is plural, does not contains->does not contain, An tree-> A tree, etc...
- Fig1: shouldn't the right-hand side of \pi contain \pi itself?
- p6: line starting with "For a production.." Check that P and matchal{P} are used correctly/
- p6: it would be so much easier to use examples instead o so many definitions.

Reaction to author response
---------------------------
The response didn't change my score.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #109B
===========================================================================

Overall merit
-------------
2. Reject - will argue against

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
Summary:
=========

The paper presents several decidable fragments of a logic that combines word equations over string variables, regular constraints (regular expressions that constrain the values of the string variables), and length constraints (Presburger formulas that constrain the length of the strings). The decision procedures for these fragments essentially follow the same methodology:

(1) computing a *reduction tree* by successively applying substitutions to a given word equation, trying to match prefixes of the left-hand and right-hand side, respectively (a boolean combination of word equations can be equivalently rewritten to a single equation). Leaves of the tree may represent equations which are trivially satisfiable (e.g., a = a) or unsatisfiable (e.g., a = b), or equations that may match inner nodes modulo a substitution. In the latter case, the leaves are connected to those inner nodes, introducing cycles. Nodes representing unsatisfiable equations are removed.

(2) unfold the cycles in the reduction tree some number of times, which depends on the regular constraints (more precisely, it depends on the number of states in the automata representing the regular languages in those constraints)

(3) remove the leaves in the unfolded tree which represent solutions of the word equation that don’t satisfy the regular constraints.

(4) transform the tree to a context-free grammar or more generally, to an EDT0L system. Let L be the language of this system.

(5) compute the Parikh image of L, and intersect it with the set of length constraints. The obtained formula is equi-satisfiable to the original formula.

The most general fragment just assumes that the reduction tree (at step 1) can be computed in finite time. A syntactically defined sub-fragment requires that the word equations are quadratic (every variable occurs at most twice). Another two fragments are defined where it is required that the tree computed at step (4) can be described by a context-free grammar.

The procedure described above is implemented and evaluated on an artificially generated benchmark. It is shown to be more precise and more efficient than other string solvers, e.g., Z3-str2, CVC4, Norn.

Strengths:
=========

- solving string constraints has numerous applications to software verification

Weaknesses:
=========

- the writing needs to be improved
- the fragments are not motivated by practical applications
- the complexity of the decision procedures is either unknown or very high (e.g., factorial)
- the experimental evaluation is weak

Evaluation:
=========

Overall, the paper is quite dense, and the quality of the writing (English) needs to be improved. Moreover, while the results seem to be correct, it is not clear whether they are relevant in practice.

The restrictions imposed to obtain decidability are quite technical and it is not clear whether they allow to solve string constraints that arise from practical applications, e.g., security issues in software manipulating strings. For instance, concerning the syntactically-defined fragments, in what context the quadratic equations are important ? Also, why it is important to even consider the fragments where the reduction tree can be represented by a context free grammar instead of an EDT0L system ? Is the Parikh image computation more efficient ?

Since the complexity of the decision procedures is either unknown or very high, the experimental evaluation is essential. And in my opinion, it would have been important to show that:
- the reduction tree computation finishes for naturally-occurring string constraints (benchmark suites can be found in the string solving literature),
- the procedure in this paper is more precise and more efficient than other string solvers on such constraints.

The artificially created benchmark used in the paper doesn’t allow to draw any useful conclusion concerning the relevance of the results. Moreover, it would have been beneficial to describe the way it was obtained, and some classification of the constraints it contains.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #109C
===========================================================================

Overall merit
-------------
4. Weak accept - will not argue for

Reviewer expertise
------------------
Z. Outsider

Paper summary
-------------
This paper presents a logic that combines word equations (s1=s2), membership in a regular language, and length constraints. The paper also presents a decision procedure for (a fragment of) this logic. Given a formula W & R & P (where W represents word equations, R represents regular expressions, and P represents Presburger arithmetic), the decision procedure works as follows: First, it constructs a reduction tree that encodes all possible solutions of W. Second, it extends (“widens”) this tree so that it encodes all solutions to W & R. Next, the algorithm transforms the tree into a finite index EDT0L system  and computes length constraints L (over Presburger arithmetic) for string variables that are implied by words accepted by the EDT0L system. The original formula W &R & P is satisfiable iff L & P is satisfiable. The paper also gives two criteria (one semantic, one syntactic) under which this procedure terminates (i.e., satisfiability is decidable).

Pros:
+ Addresses an important problem
+ Introduces novel ideas (to the best of my knowledge)
+ Contains useful theoretical results

Cons:
- Some parts of the paper are not well-written and hard to understand
- Experimental evaluation is on artificial benchmarks (although the results on those benchmarks look good)

Comments for author
-------------------
I think this paper addresses a very important problem -- determining satisfiability of the logic presented in this paper has many real-world applications (e.g., static analysis for security properties). Hence, I'm sympathetic towards the problem that this paper is tackling. To the best of my knowledge, the techniques presented in the paper are also novel, and, overall, I found the results presented in the paper interesting.

My main criticism is that the paper fails to provide intuition about the necessity of various moving parts. In particular, why is it necessary to convert the tree to the EDT0L system? Also, I had no background in this topic, and the background provided in the paper is not sufficient to follow all the details. For instance, the authors could make the rest of the paper much more readable by giving some examples in 2.2. Given that most of the POPL attendees are unlikely to be experts in this topic, I think most readers may have the same problem.

The experimental evaluation makes the proposed approach look quite favorable compared to existing solvers, but it seems that the evaluation is performed on artificial formulas. Can you elaborate on how these formulas were generated during the rebuttal? Why did you not compare against existing tools on benchmarks used in prior work? I would have found the experiments much stronger if the benchmarks had some relevance to real-world problems.

Another complaint is that the paper is a bit distracting because it constantly interleaves the technical description of your technique with comparison against related work (e.g., third paragraph in intro, paragraph before contributions in intro,”We remark that Makanin's algorithm ...” on page 9 etc.) The paper would read much better if you include such discussions in related work and not intersperse them throughout the paper.
Other questions/comments:

- Can you comment on how to obtain a model using your decision procedure during the rebuttal?
- You keep saying that you “partially implemented a prototype”. What does it mean to “partially implement” the solver? Please clarify during rebuttal.
- In Fig 1, why do you restrict yourself to only DNF formulas? (not quite DNF, but disjunctions on the outside)
- The terminology on page 4 is a bit confusing. For instance. Why do you call the word equation “acyclic” rather than “linear”? Can you give some intuition about the terminology “twisted” and why you are introducing it here?
- You *really* need to give some examples to illustrate EDT0L in Section 2.2.
- There is a very confusing typo in definition of “deterministic ET0L” (what is the exclamation mark?)
- Section 2.3: define semilinear set
- Section 3.1: what is a “virtual cycle”?
- In 3.2, it was not clear what you meant by “complete cases” – you should explain.
- Page 8, last paragraph: “Pakikh” => Parikh
- Please add references to proofs of lemmas.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #109D
===========================================================================

Overall merit
-------------
2. Reject - will argue against

Reviewer expertise
------------------
X. Expert

Paper summary
-------------
This paper studies (decidability of) satisfiability of word equations
combined with regular expression constraints and length
constraints. The paper introduces a new paradigm for constructing
decision procedures, based on the notion of a reduction tree that is
obtained from word equations by systematic splitting; from such
reduction trees it is then possible to extract constraints about the
length of solution words in Presburger arithmetic. The paper claims
that this procedure can decide satisfiability of quadratic word
equations (equations in which each variable occurs at most twice)
combined with regular expression constraints and length constraints
(Theorem 5.20; Def 10), which would solve a longstanding open problem
in CS.

There seems to be a fundamental flaw in the paper, however; I'm not
entirely sure at which point the paper goes wrong, but it seems that
the overall procedure just cannot work due to basic results about word
equations.

The general approach to decide satisfiability of a conjunction
E & R & alpha (where E is a word equation, R are regex constraints,
and alpha are length constraints in Presburger arithmetic) is as
follows (see p3, p14):

* the equation E is expanded to a finite, cycle reduction tree T1
  representing all solutions of E

* the tree T1 is extended to a tree T2, also taking the regex
  constraints R into account

* from T2, a Presburger formula alpha_w is extracted that precisely
  describes lengths of words satisfying E & R (let's call alpha_w the
  "length abstraction" of E & R)

* satisfiability of the conjunction alpha_w & alpha is checked

However, it is known that the length abstraction of word equations
combined with regex constraints (even in the quadratic case) is in
general /not/ semi-linear; i.e., it cannot always be defined in
Presburger arithmetic. This indicates that somewhere on the way of
computing alpha_w there has to be a mistake.

As an example, consider the conjunction

(1)  A.B = B.A &

(2)  A \in \Sigma* a \Sigma* &

(3)  B \in \Sigma* b \Sigma*

It is well-known that the quadratic word equation (1) is satisfied for
words A, B iff there is a word C such that A = C^n and B = C^m; in
other words

    A.B = B.A iff (exists C. A \in C* & B \in C*)

(for instance, see Theorem 3 in "Combinatorics of words", Juhani
Karhumäki,
https://www.utu.fi/en/units/sci/units/math/staff/Documents/karhumaki/combwo.pdf)

(2) and (3) imply that the C needs to have length >= 2, since it has
to contain characters a and b. The length abstraction of (1) & (2) &
(3) is therefore

    |A| >= 1 & |B| >= 1 &
    exists k. k >= 2 & (k divides |A|) & (k divides |B|)

But this is a relation between |A| and |B| that cannot be represented
in Presburger arithmetic!

Note that the counterexample does not show undecidability of quadratic
word equations + regex constraints + length constraints (this is still
an open problem), but that the path proposed in the paper has to be
revised.

Comments for author
-------------------
The names STR_EDT0L and STR^dec_EDT0L for different fragments of the
considered logic are rather unintuitive (e.g., STR_EDT0L is the name
for quadratic word equations).

The transformation of equations on p10/11 is essentially Nielsen's
transformation, [15].

Some typos:

Norm -> Norn

PSPASE -> PSPACE

p2 "may not in a"

p3 "we are the first one to present a decidability result for a
fragment of string logic including the whole fragment of Presburger
arithmetic over the lengths" arguably, this has already been done in
[2] and [36], among others

p7, in the definition of reduction trees the elimination of common
prefixes of lhs and rhs is not handled very cleanly


==> syntax-dp.tex <==
\begin{algorithm}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$(s, \ses)$}\Output{G}
   $G {\leftarrow}  \code{vertex}(s)$;$WL {\leftarrow} \{s\}$\;
 \While { $WL{\not=}\emptyset$ }
 {
    $s_i {\leftarrow}  \code{head}(WL)$;$WL {\leftarrow}  \code{tail}(WL)$\;
    $\code{is\_exist}, tr_i,tr_d,\ses {\leftarrow} \code{choose\_intersect}(s_i,\ses)$\;
    \uIf{\code{is\_exist}}{
      \uIf{$\FV(tr_d)==\emptyset$}{
        \ForEach{$s_j$ $\in$ $\FV(tr_i)$ }{
          $G {\leftarrow}  \code{vertex}(s_j)$\;
          \tcc{mark $s_j$ as leaf}
        }
       }
      \uElse{
         \ForEach{$s_j$ $\in$ $\FV(tr_d)$ }{
          $G {\leftarrow}  \code{vertex}(s_j)$;
          $G {\leftarrow}  \code{edge}(s_i,s_j)$;
          $WL {\leftarrow} WL {\cup} \{ s_j\}$\;
         }
      }
    }
    \uElse{ %%({\em /* mark $s_i$ as leaf */})
      \tcc{mark $s_i$ as leaf}
    }
 }
 \caption{Dependency Graph Construction}\label{algo.dp}
\end{algorithm}


==> tree-2-cfg.tex <==
\input{fig-cfg}
We describe a novel procedure, called \form{\extractcfg},
to transform a cyclic reduction tree
derived by {\allSat} for a word equation over \form{\stredtsem},
into a CFG.
Intuitively, given a cyclic reduction tree \form{\utree{i}}
with the root \form{\form{\se_r}}
all solutions of \form{\se_r}
are obtained from the solution traces, each of which
 corresponds to a path starting
 from the root
and ending
 with a satisfiable leaf node.
Intuitively,
each path ending with a satisfiable leaf node which is not involved in any back-link represents
(a way to derive) a solution which can be obtained by splitting the string variables
according to the edges in the path. A cycle in the tree thus represents an infinite set of
solutions, since we can construct infinitely many paths by iterating through the cycle an
unbounded number of times.
Therefore, if a solution trace (corresponding to a satisfiable leaf node) includes
 (either directly or indirectly) with
some cycles, procedure \form{\extractcfg}
  additionally
collects those traces from
these cycles.
A trace collected from
a solution trace
with cycles represents
a {\em family} of infinite solutions of the root.

\input{algo-flaten}
Procedure \code{\extractcfg} is described in
Algorithm \ref{algo.cfg}.
To compute a CFG
 for a cyclic tree, procedure \code{\extractcfg}
computes a CFG for each solution trace
using an auxiliary procedure \code{\extractaux} (line 3).
Function \code{sat\_leaf(\utree{i})} returns
a set of satisfiable leaf nodes of the tree \code{\utree{i}};
procedure \code{\extractaux(\se_r, \se_i)} returns
a pair of  variables and production rules
in the solution trace from the root \form{\se_r} to
the satisfiable leaf node \form{\se_i}.
For each solution trace, we add
one new start symbol \form{S_i} (\form{S_i} is a fresh variable)
and its rule (line 4) to indicate that
the language includes all sentences
of the left-hand side of the root
\form{\se_r}. Note that \code{LHS(\form{\se})}
returns the left-hand side of equation \form{\se}.
After generating CFGs for all solution traces,
it unions all these CFGs to form the set of
all solutions (line 7).


Procedure  \code{\extractaux} is presented
in Algorithm \ref{algo.ftree}. It takes a 
solution path \form{(\se_r, \se_i)} as input and generates
a pair of the set of variables \form{\var_i}
and the set of productions \form{\productions_i}.
%This procedure
 \code{\extractaux} works as follows.
First, it collects a sequence of all cycles (line 1),
labels (a.k.a substitutions) of edges which do not involve in any cycle (line 2)
and the set of variables (line 3).
We note that the sequence of all cycles is sorted in
a top-down manner.
The cycle
\form{\ctree{\se_{c_i}}{\se_{b_i}}{\sub_{cyc_i}}}
is sorted so as it stands before the 
 \form{\ctree{\se_{c_j}}{\se_{b_j}}{\sub_{cyc_j}}}
if the companion node \form{\se_{c_i}}
is closer to the root than the companion node \form{\se_{c_j}}.
Function \code{labels} is used at line 2 (and line 18)
to collect all labels of a path or a cycle (including the
label in the back-link).
After that,  at lines 6-15 \code{\extractaux} collects
production rules
for each variable. In general,
along a path from the root to a satisfiable leaf node
a variable \form{X} may be extensible from
\form{k} cycles (\form{k\geq0}), say
\form{\vtree{\se_{c_1}}{\se_{b_1}}{\sub_{cyc_1}}{X}},
..., and \form{\vtree{\se_{c_k}}{\se_{b_k}}{\sub_{cyc_k}}{X}},  prior to being substituted.
To generate valid solutions, it is required to
 split extensible variables
through cycles in the same order as they appear in the tree.
To do that, we introduce a sequence of auxiliary staged variables.
For instance, for the above variable \form{X} we introduce fresh variables
\form{\{X_1, ..., X_k \}}
  each of which represents for \form{X} at a cycle.
In Algorithm \ref{algo.ftree},
staged variables are introduced at lines 5-16.
The auxiliary procedure \form{\ulabels{Obj}{\sub        }}
is used to apply the substitutions \form{\sub}
into the object \form{Obj}.
The object could be either
a cycle at line 9 or a set of substitutions at line 14.
We remark that at line 10 we add production rules
to connect cycles wrt. an extensible variable
 together.
Afterward, \code{\extractaux} collects production
rules from labels (substitutions)
of cycles (line 18) and non-cyclic path (line 20).

\begin{example}
We illustrate procedure \code{\extractcfg}
through the example in Fig. \ref{fig.red.complex.tree3}.
In this example, we generate a CFG for the
solution trace of the path \form{(\se_0, \se_9)}.
\input{min-tree2}
While the input is on the left which is involved in three cycles
(two extended for \form{x} and one extended for \form{y}),
the staged variables (\form{\{X_1, X_2, Y_1\}})
 have been added as in the tree on the right.
The production rules generated is:
\[
\begin{array}{c|c}
x & y \\
\hline
\begin{array}{ll}
\begin{array}{l}
 \form{ x \rightarrow yx_1} \\
 x_1 \rightarrow x
\end{array} & \text{//$1^{st}$ cycle on } x \\
\form{x \rightarrow X_1} & \text{//connect to $2^{nd}$ cycle on } x \\
\begin{array}{l}
 \form{ X_1 \rightarrow y_1x_2} \\
 x_2 \rightarrow X_1
\end{array} & \text{//$2^{nd}$ cycle on } x \\
\form{X_1 \rightarrow X_2} & \text{//connect to non-cycle on } x \\
\form{X_2 \rightarrow \semp} & \text{//non-cycle on } x \\
\end{array}
 &
%%%%%%%%%%%%%%%%%%%%%%%
\begin{array}{ll}
\begin{array}{l}
 \form{ y \rightarrow xy_1} \\
 y_1 \rightarrow cy_2 \\
y_2 \rightarrow y
\end{array} & \text{//$1^{st}$ cycle on } y \\
\form{y \rightarrow Y_1} & \text{//connect to non-cycle on } y \\
\form{Y_1 \rightarrow X_1y_1} &   \text{//non-cycle on } y \\
\form{y_1 \rightarrow \semp} & \text{//non-cycle on } y \\
\end{array}
\end{array}
\]
\end{example}

\paragraph{Correctness}
%% In the rest of this subsection, we show
%% the correctness of function {\extractcfg}.
By construction, procedure \form{\extractaux}
capture all solutions of the solution path.
As context-free languages are closed under union \cite{Hopcroft:2006:IAT},
{\extractcfg} produces a CFG.
\begin{cor}\label{thm.cfg}
The reduction tree of
a solvable word equation \form{\se}
over \form{\strcfsem}
forms a {\cfl}%% context-free language
.
\end{cor}
%% \begin{proof}

%% \qed
%% \end{proof}


==> tree-term.tex <==
%%for termination
In this subsection,
 we show the termination of {\allSat} for quadratic
systems.
As so, we can made use of {\allSat} as a decision
procedure for quadratic systems as follows.
Given a quadratic equation \form{\se},
we first use  {\allSat} to construct for it
a cyclic reduction tree.
After that, we check whether there exists
a satisfiable leaf node in the tree.
If it is the case, we return {\sat}.
Otherwise, we return {\unsat}.

For the termination of \form{\allSat} on
 quadratic word equations,
we first show a weak form of the computation complexity
as follows.
The proof of this result replies on the following Lemma.
\begin{lemma}\label{lem.reduce.size}
Let \form{\code{L{=}\transform}(\se(N))}. Then,
for each \form{(\se'(N'), \sub) \in L},
  \form{N'{\leq}N}.
\end{lemma}
\begin{proof}

\qed
\end{proof}

\begin{lemma}[Weak]\label{lemma.allsat.compl}
Let \form{\se(N)} 
 be a quadratic word equation.
The length of every path in the (sub-)tree whose root is \form{\se(N)}
is $\mathcal{O}(N^2(N!))$.
\end{lemma}
\input{proof-all-sat-term}

polynomial algorithm
\begin{lemma}\label{lem.reduce.cycle}
Length of a cycle is less than word equation length.
\end{lemma}

\begin{proof}
One occurrence.

We remark that a cycle is constructed when the equation at the root of the tree
contains at least one variable with two occurrences.

If two occurrences are at the same side

one is in LHS and another is in RHS.
Without loss of general, assume that the companion of a cycle
of variable \form{X} is
\form{X tr_1 = Ytr_2 X}. At the first reduction,
\form{YX_1/X}, \form{X_1 tr_1 = tr_2 YX_1}.  To form a cycle,
at each reduction step, the first term (a variable or a character)
in the LHS
is reduced and matched with the first term in the RHS
until \form{Y} variable is the first term of the RHS.
so, the length of the cycle is equal to \form{N{-}1}.
\end{proof}

\begin{lemma}\label{lem.reduce.min.sol}
Minimal solution is polynomial
\end{lemma}

\begin{proof}
max \form{N/2} cycles

\form{(N/2) \times (N-1) + N}
\end{proof}

\begin{proposition}[{\allSat} Termination]\label{lemma.allsat.term}
{\allSat} terminates for quadratic word equations.
\end{proposition}

\begin{proof}
The correctness of this
 proposition immediately follows from lemmas \ref{lem.reduce.size}
and \ref{lemma.allsat.compl}.
\qed
\end{proof}


==> weq.tex <==
 %% \begin{figure}[tbh]
 %% \begin{center}
 %% \begin{minipage}{0.98\textwidth}
 % \begin{frameit}

 \begin{algorithm}[t]
%%\begin{procedure}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$\ind$} \Output{\utree{n}}
   $i {\leftarrow} 0 $; %% $\sstate^{comp} {\leftarrow} \{ \}$;
   %% $\sstate {\leftarrow} \{ \ind \}$ \tcc*{initialize}
   $\utree{0} {\leftarrow} \{ \ind \}$ \tcc*{initialize}
 \While { $\true$ }
 {
      $\utree{i} {\leftarrow} \code{\oo}(\utree{i})  $ \tcc*[r]{marked unsat and closed}
      $ \utree{i}  {\leftarrow} \code{isomorphic}(\utree{i}) $ \tcc*[r]{detect similarly}
      $(\code{is\_exists}, \ind_i) {\leftarrow} \code{choose\_bfs}(\utree{i})  $ \tcc*[r]{open leaf for unfolding}
      \uIf{ not~ \code{is\_exists}}{
       \Return{\utree{i}};
     }\Else{
        $ i {\leftarrow} i{+}1 $ \;
       $ \utree{i}  {\leftarrow} \code{unfold}(\ind_i) $\;
      }
 }
 \caption{Constructing Periodic Trees.}\label{algo.periodic.tree}
\end{algorithm}
%\savespace
%%\end{procedure}

